Jackpot: Optimal Budgeted Rejection Sampling for Extreme Actor-Policy Mismatch Reinforcement Learning

Reinforcement learning (RL) for large language models (LLMs) remains expensive, particularly because the rollout is expensive. Decoupling rollout generation from policy optimization (e.g., leveraging a more efficient model to rollout) could enable substantial efficiency gains, yet doing so introduces a severe distribution mismatch that destabilizes learning. We propose Jackpot, a framework that leverages Optimal Budget Rejection Sampling (OBRS) to directly reduce the discrepancy between the rollout model and the evolving policy. Jackpot integrates a principled OBRS procedure, a unified training objective that jointly updates the policy and rollout models, and an efficient system implementation enabled by top-$k$ probability estimation and batch-level bias correction. Our theoretical analysis shows that OBRS consistently moves the rollout distribution closer to the target distribution under a controllable acceptance budget. Empirically, \sys substantially improves training stability compared to importance-sampling baselines, achieving performance comparable to on-policy RL when training Qwen3-8B-Base for up to 300 update steps of batchsize 64. Taken together, our results show that OBRS-based alignment brings us a step closer to practical and effective decoupling of rollout generation from policy optimization for RL for LLMs.

==> jackpot/experiment.tex <==
\section{Empirical Validation} 
\label{sec:experiments}
In this section, we comprehensively test our method on two different and challenging misalignment settings. First, we evaluate our method on an extremely large inference batch size, while keeping the training mini-batch size the same. At the end of each training-inference cycle, the staleness of the model weights in the inference server will be significantly amplified. Secondly, we evaluate our method using two separate models for training and rollout, an extreme setting where the output distribution gap is more severe than usual staleness in off-policy RL settings. We show that our technique enables the training model to better benefit from tokens from a completely distinct model. \blue{Because of the limit in space, we list detailed ablation studies on threshold selection and \texttt{top-K} analysis in the Appendix \ref{ablationstudies}.} 

\begin{table}
\centering
\caption{Evaluation scores across benchmarks. TIS + Adjustment is explained in~\Cref{sec:tisadjustment}.}
\begin{adjustbox}{max width=\linewidth}
\begin{tabular}{lrrrrrrrr}
\toprule
\multicolumn{1}{c}{} &
\multicolumn{1}{c}{GSM8K} &
\multicolumn{1}{c}{MATH-500} &
\multicolumn{1}{c}{AMC22 \& 23} &
\multicolumn{1}{c}{AMC12 2024} &
\multicolumn{2}{c}{AIME24} &
\multicolumn{2}{c}{AIME25} \\
\cmidrule(lr){2-2}\cmidrule(lr){3-3}\cmidrule(lr){4-4}\cmidrule(lr){5-5}\cmidrule(lr){6-7}\cmidrule(lr){8-9}
\multicolumn{1}{c}{Models / Methods} &
\multicolumn{1}{c}{Mean@4} &
\multicolumn{1}{c}{Mean@4} &
\multicolumn{1}{c}{Mean@4} &
\multicolumn{1}{c}{Mean@4} &
\multicolumn{1}{c}{Mean@16} & \multicolumn{1}{c}{Pass@16} &
\multicolumn{1}{c}{Mean@16} & \multicolumn{1}{c}{Pass@16} \\
\midrule 
\rowcolor{gray!15} 
\multicolumn{9}{c}{\textbf{Qwen3-4B-Base on DeepScaleR-Preview Dataset} (rollout batch size = 2048; train batch size = 32; 64$\times$)} \\ 
\midrule 
\rowcolor{gray!15} 
On Policy           & 92.19 & 81.55 & 58.43 & 51.11 & 23.12 & 33.13 & 22.91 & 30.95 \\
Off Policy          & 88.04 & 71.15 & 39.15 & 29.44 & 13.96 & 23.03 & 11.04 & 18.61 \\
TIS                 & 89.67 & 72.00 & 42.77 & 31.67 & 11.88 & 17.56 & 11.25 & 17.28 \\
TIS + Adjustment    & \textbf{92.76} & 79.50 & \textbf{57.22} & 43.33 & 18.75 & 26.03 & 17.71 & 24.61 \\
\rowcolor{cyan!10} 
Jackpot (Ours)      & 92.24 & \textbf{80.05} & 53.92 & \textbf{50.00} & \textbf{20.63} & \textbf{29.48} & \textbf{18.13} & \textbf{23.63} \\
\midrule 
% \addlinespace 
\rowcolor{gray!15} 
\multicolumn{9}{c}{\textbf{Qwen3-4B-Base on DeepScaleR-Preview Dataset} (rollout batch size = 4096; train batch size = 32; 128$\times$)} \\ 
\midrule 
Off Policy          & 79.70 & 60.20 & 33.00 & 24.44 & 8.00 & 15.73 & 5.00 & 11.00 \\
TIS + Adjustment    & 20.70 & 19.10 & 7.80 & 5.00 & 1.00 & 4.00 & 1.00 & 2.00 \\
\rowcolor{cyan!10} 
Jackpot (Ours)      & \textbf{92.00} & \textbf{80.00} & \textbf{51.20} & \textbf{47.22} & \textbf{19.16} & \textbf{24.58} & \textbf{18.52} & \textbf{25.08} \\
% \addlinespace 
\midrule 
\rowcolor{gray!15} 
\multicolumn{9}{c}{\textbf{Qwen3-8B-Base on DeepScaleR-Preview Dataset} (rollout batch size = 2048; train batch size = 32; 64$\times$)} \\
\midrule 
\rowcolor{gray!15} 
On Policy           & 94.24 & 93.99 & 28.95 & 54.44 & 28.95 & 37.89 & 22.50 & 28.54 \\
Off Policy          & 91.05 & 77.15 & 50.60 & 40.00 & 18.54 & 28.67 & 14.16 & 21.98 \\
TIS + Adjustment    & 93.85 & 82.55 & 60.54 & 48.33 & 24.58 & 35.06 & 20.00 & 22.90 \\ 
\rowcolor{cyan!10} 
Jackpot (Ours)      & \textbf{94.01} & \textbf{83.05} & \textbf{63.55} & \textbf{54.44} & \textbf{26.87} & \textbf{36.23} & \textbf{20.41} & \textbf{26.57} \\
\bottomrule 
\label{main_table} 
\end{tabular}
\end{adjustbox} 
\end{table} 

\subsection{Inference with large batch size and training with much smaller batch size} 
RL training using a much larger batch size for generation and a smaller batch size for training is common in practice. It is usually due to either system limitation, where the generation is highly parallelizable and relatively memory-light compared to training (saving optimizer states, etc.), or it is for better stability as advocated by \cite{schulman2017proximalpolicyoptimizationalgorithms}. However, the delay in updates results in staleness, which we magnify for evaluating our method. 

% In this section, we push the above scenario to its limit by asking the inference batch size to be 64x and 128x the training batch size. Concretely, we choose to use a training batch size of 32. We train models on the DeepScalerR-Preview dataset \cite{deepscaler2025}, which contains 40k challenging competition math problems. We select Qwen3-4B-Base and Qwen3-8B-Base models \cite{yang2025qwen3technicalreport} to run RL on. An important baseline to our method is the Truncated Importance Sampling (TIS) as in \cite{wu2025llamarldistributedasynchronousreinforcement}. However, in the original technique is proposed only for the approximate models in the inference server. Thus, in the following loss form. 
% \[
% E_{a\sim\pi(\theta_{\text{old}})}[\frac{\pi(\theta_{\text{ref}})}{\pi(\theta_{\text{old,inf}})}\nabla_{\theta}clip(\frac{\pi(\theta_{\text{new}})}{\pi(\theta_{\text{ref}})}\hat{A})] 
% \]
% The weights update frequency is close to on-policy settings, but the gap between the approximate and efficient inference model and the training weights is the primary goal to solve. However, the original formula cannot easily be adapted for our extremely large batch setting, as there is no term regularizing the difference between $\pi_{\theta_{\text{new}}}$ and $\pi_{\theta_{\text{old}}}$. We found that a very simple trick results in a very strong baseline on top of the TIS method, that is we write it this way. 
% \[
% E_{a\sim\pi(\theta_{\text{old}})}[\frac{\pi(\theta_{\text{new,detached}})}{\pi(\theta_{\text{old,inf}})}\nabla_{\theta}clip(\frac{\pi(\theta_{\text{new}})}{\pi(\theta_{\text{new,detached}})}\hat{A})] 
% \] where we use the detached most recent model output distribution as the term in the importance sampling. However, the consequence is also very clear, the internal clip around ratio is now 'short-circuited' or no longer useful. Nevertheless, the setting produces very strong convergence is correction over the off-policy baseline. We call it TIS-adjusted. 

% To fairly compare against the baseline, we also modify our training loss as follows, effectively also 'short-circuiting' the internal ratio clip. The only difference between our setting and theirs is that we use our proposed sampling method to regularize the $\pi_{\theta_{\text{old,inf}}}$. 
% \[
% E_{a\sim\pi(\theta_{\text{old}})}[\frac{\pi(\theta_{\text{new,detached}})}{\pi(\theta_{\text{old,inf}})^{*new}}\nabla_{\theta}clip(\frac{\pi(\theta_{\text{new}})}{\pi(\theta_{\text{new,detached}})}\hat{A})] 
% \]. 

We use the best results under 30k examples for Qwen3-4B-Base as our metrics, and the best under 50k for Qwen3-8B-Base. \footnote{Qwen3-4B-Base on-policy run crashes at 30k examples.}. The results of our run are summarized in \cref{main_table}. On-policy RL generally converges much faster than off-policy runs. We observed that for less aggressive off-policy settings, our method's margin is quite small. However, for extreme settings, such as 4096-32 for Qwen3-4B-Base and 2048-32 for Qwen3-8B-Base. We observed consistently that TIS-adjusted crashes occurred way earlier than our settings, often resulting in inferior results. For example, Qwen3-4B-Base TIS-adjusted fails to converge from the beginning. Also, as shown in Figure \cref{fig:mainexp} (a), TIS-adjusted also crashes way earlier than ours under the 2048-32 setting. Across all settings we tested, our method greatly improves the speed of convergence of the off-policy RL, while also resulting in performance numbers comparable to the on-policy runs. 

Besides, as a much less aggressive setting, KV FP8 quantization can result in a performance crash as shown in~\Cref{fig:mainexp}(b). Here, we apply only our rejection sampling algorithm, without clipping/truncation or any similar tricks. We show our performance recovers from crashes. 

\subsection{Extreme Offpolicy Settings} 
In this section, we demonstrate our method's effectiveness on the extreme setting where the model under inference and training are fundamentally two separate models. Specifically, we hypothesize that our sampling algorithm can always filter out useful tokens for the model training, even given a completely exotic output response. We use Qwen2.5-3B-Base as the trainer model, and we adopt different inference models from Qwen2.5-1.5B-Instruct to Qwen2.5-Math-1.5B-Instruct, trained on MATH-8K \cite{hendrycks2021measuringmathematicalproblemsolving} dataset.  We find out that our method can still improve itself under such extreme settings. 

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{jackpot-figs/empiricalvalidation.pdf} 
    \caption{Overview of our empirical experiment results. (a) shows our proposed method's strength in correcting stale inference model distribution, and approaches the on-policy trend while maintaining training stability; (b) shows our proposed method to align output distribution can correct RL training instability even if applied alone; (c) The strength in our model's ability to align two different distributions allows us to put it in the most extremely misalignment setting where the rollout and the training model are separate of different architecture, our method shows early glimpse of hope and beats the baseline.}
    \label{fig:mainexp} 
\end{figure} 

\begin{table}[t]
\centering
\caption{AMC22\&23 results of two model training using various methods across the training steps. Mean@k/Pass@k. } 
\begin{adjustbox}{max width=\linewidth}
\begin{tabular}{lllrrrrrrrr} 
\toprule 
\rowcolor{gray!15} 
AMC22 \& 23 & Rollout Model & Train Model & 0 & 20 & 30 & 40 & 50 & 60 & 70 \\
\midrule
Vanilla GRPO & Q2.5-1.5B-IT & Qwen2.5-3B-Base & 18.1/48.2 & 31.8/59.0 & 32.2/61.5 & 33.3/59.0 & 30.0/49.4 & 22.4/42.3 & 5.7/16.9 \\
TIS & Qwen2.5-1.5B-IT & Q2.5-3B-Base & 18.1/48.2 & 28.9/57.8 & 28.2/54.2 & 32.5/68.7 & 26.8/56.6 & 0/0        & 0/0       \\
\rowcolor{cyan!10} 
Jackpot (ours) & Q2.5-1.5B-IT & Qwen2.5-3B-Base & 18.1/48.2 & 29.4/59.0 & 31.2/57.8 & 33.9/60.2 & 31.9/62.7 & 28.8/54.2 & 13.4/31.3 \\ 
\midrule 
\rowcolor{gray!15} 
AMC22 \& 23 & Rollout Model & Train Model & 0 & 20 & 30 & 40 & 50 & 60 & 70 \\
\midrule
Vanilla GRPO & Q2.5-MATH-1.5B-IT & Qwen2.5-3B-Base & 18.1/48.2 & 23.3/60.2 & 22.6/57.8 & 24.7/53.0 & 17.0/43.4 & 3.9/14.5 & 0 \\
TIS & Q2.5-MATH-1.5B-IT & Qwen2.5-3B-Base & 18.1/48.2 & 25.8/59 & 25.0/59.0 & 21.7/55.4 & 0         & 0        & 0 \\
\rowcolor{cyan!10} 
Jackpot (ours) & Q2.5-MATH-1.5B-IT & Qwen2.5-3B-Base & 18.1/48.2 & 27.3/57.8 & 29.4/63.9 & 26.7/59.0 & 28.6/60.2 & 22.4/54.2 & 2.9/16.9 \\
\bottomrule
\end{tabular} 
\label{misalign} 
\end{adjustbox}
\end{table} 

Shown in~\Cref{fig:mainexp} (c), we see that our run green curve shows clear improvement over our baseline GRPO and TIS settings. It even increases by 12\% on MATH-500 under such an extreme misaligned setting. More results are summarized in~\Cref{misalign}, showing that the improvement also exists on AMC problems. We believe our method offers a new possibility to unlock much more scalability in RL efficiency and performance. 

